Cluster Aggregated GAN (CAG): A Cluster-Based Hybrid Model for Appliance Pattern Generation

Synthetic appliance data are essential for developing non-intrusive load monitoring algorithms and enabling privacy preserving energy research, yet the scarcity of labeled datasets remains a significant barrier. Recent GAN-based methods have demonstrated the feasibility of synthesizing load patterns, but most existing approaches treat all devices uniformly within a single model, neglecting the behavioral differences between intermittent and continuous appliances and resulting in unstable training and limited output fidelity. To address these limitations, we propose the Cluster Aggregated GAN framework, a hybrid generative approach that routes each appliance to a specialized branch based on its behavioral characteristics. For intermittent appliances, a clustering module groups similar activation patterns and allocates dedicated generators for each cluster, ensuring that both common and rare operational modes receive adequate modeling capacity. Continuous appliances follow a separate branch that employs an LSTM-based generator to capture gradual temporal evolution while maintaining training stability through sequence compression. Extensive experiments on the UVIC smart plug dataset demonstrate that the proposed framework consistently outperforms baseline methods across metrics measuring realism, diversity, and training stability, and that integrating clustering as an active generative component substantially improves both interpretability and scalability. These findings establish the proposed framework as an effective approach for synthetic load generation in non-intrusive load monitoring research.

==> figs/fig1/panel_a.tex <==
% ---------------------------------------------------------------------
% Fig. 1 (a): measured vs. generated windows, two appliances x four models.
% Every curve is real data, emitted by code/scripts/fig1_data.py into
% traces.tex. Coverage values are the per-device numbers behind Table 3;
% regenerate both with the scripts in code/scripts/ if the results change.
% Local frame: origin at the panel's bottom-left, 10.05 x 4.60 units.
% ---------------------------------------------------------------------
\begin{scope}
  \def\cw{2.22}   % cell width
  \def\ch{1.24}   % cell height
  \def\gx{0.16}   % gap between columns
  \def\lx{0.66}   % width of the left row-label strip

  \node[ptitle] at (0,4.40) {(a) Measured and generated appliance windows};
  \node[psub]   at (0,4.14)
    {three windows per cell; the number below each cell is that model's $k$-NN Coverage};

  % ---- column headers ----
  \foreach \i/\t/\s in {0/Measured/{UVIC}, 1/BehaviorGAN/{baseline},
                        2/CNN-GAN/{baseline}, 3/\textbf{CAG}/{ours}} {
    \node[lab, anchor=south] at ({\lx+\i*(\cw+\gx)+\cw/2}, 3.78) {\t};
    \node[font=\cgtiny, text=cgSlate, anchor=north]
      at ({\lx+\i*(\cw+\gx)+\cw/2}, 3.76) {\s};}

  % ---- the eight cells --------------------------------------------------
  % row 0 = WaterCooler, intermittent, so its CAG cell takes the branch blue
  % row 1 = Refrigerator, continuous, so its CAG cell takes the branch green
  \foreach \r/\dev/\tag/\accent/\covb/\covc/\covd in {%
      0/WaterCooler/WC/cgBlue/0.000/0.157/0.321,
      1/Refrigerator/RF/cgGreen/0.122/0.000/0.725} {
    % per row: which baseline collapses here, and the branch colour of CAG
    \ifnum\r=0
      \def\chipbeh{chipA}\def\txtbeh{collapsed}\def\chipcnn{chipN}\def\txtcnn{duty high}%
      \def\chipcag{chipB}\def\txtcag{shape kept}%
    \else
      \def\chipbeh{chipN}\def\txtbeh{envelope lost}\def\chipcnn{chipA}\def\txtcnn{collapsed}%
      \def\chipcag{chipG}\def\txtcag{modes kept}%
    \fi
    \pgfmathsetmacro{\yb}{2.26-\r*1.60}
    \node[lab, rotate=90] at (0.14,{\yb+\ch/2}) {\dev};
    \foreach \i/\key/\col/\cov/\vchip/\vtxt in {%
        0/real/cgSlate/{}/chipN/{},
        1/beh/cgGrey/\covb/\chipbeh/\txtbeh,
        2/cnn/cgGrey/\covc/\chipcnn/\txtcnn,
        3/cag/\accent/\covd/\chipcag/\txtcag} {
      \pgfmathsetmacro{\xl}{\lx+\i*(\cw+\gx)}
      \draw[well] (\xl,\yb) rectangle ({\xl+\cw},{\yb+\ch});
      \begin{scope}
        \clip (\xl,\yb) rectangle ({\xl+\cw},{\yb+\ch});
        \begin{scope}[shift={(\xl,\yb)}, x=\cw cm, y=\ch cm,
                      trace/.append style={draw=\col}]
          \csname cell\tag\key\endcsname
        \end{scope}
      \end{scope}
      % tag and verdict both live under the cell: nothing is drawn on top of
      % the data, so the reader compares waveforms without an obstruction
      \ifx\cov\empty
        \node[font=\cgtiny, text=cgSlate, anchor=north east, inner sep=1.6pt]
          at ({\xl+\cw},\yb) {measured};
      \else
        \node[font=\cgtiny, text=cgSlate, anchor=north east, inner sep=1.6pt]
          at ({\xl+\cw},\yb) {\cov};
        \node[\vchip, anchor=north west, inner xsep=2pt, inner ysep=1pt]
          at ({\xl+0.02},{\yb-0.02}) {\vtxt};
      \fi}}

\end{scope}


==> figs/fig1/panel_b.tex <==
% ---------------------------------------------------------------------
% Fig. 1 (b): the realism-diversity plane, averaged over the eleven
% appliances. Coordinates are the (MMD, Coverage) columns of Table 2;
% regenerate with code/scripts/gen_paper_tables.py and update here.
% Local frame: origin at the panel's bottom-left, 5.30 x 4.60 units.
% ---------------------------------------------------------------------
\begin{scope}
  \def\px{1.00}\def\py{1.46}\def\pw{4.05}\def\ph{2.26}
  \def\mmdmax{0.50}\def\covmax{0.58}
  % MMD runs right-to-left, so "better on both axes" is up and to the right
  \newcommand{\pt}[2]{({\px+(\mmdmax-#1)/\mmdmax*\pw},{\py+#2/\covmax*\ph})}

  \node[ptitle] at (0,4.40) {(b) Realism against diversity};
  \node[psub]   at (0,4.14) {mean over the eleven appliances};

  \draw[well] (\px,\py) rectangle ({\px+\pw},{\py+\ph});
  \foreach \c in {0.2,0.4} {
    \draw[lane] (\px,{\py+\c/\covmax*\ph}) -- ({\px+\pw},{\py+\c/\covmax*\ph});
    \node[font=\cgtiny, text=cgSlate, anchor=east, inner sep=2pt]
      at (\px,{\py+\c/\covmax*\ph}) {\c};}
  \foreach \m in {0.1,0.2,0.3,0.4} {
    \draw[lane] \pt{\m}{0} -- \pt{\m}{\covmax};
    \node[font=\cgtiny, text=cgSlate, anchor=north, inner sep=2pt] at \pt{\m}{0} {\m};}
  \node[font=\cgtiny, text=cgSlate, anchor=north] at ({\px+\pw/2},{\py-0.22})
    {MMD $\downarrow$ (realism, better $\rightarrow$)};
  \node[font=\cgtiny, text=cgSlate, rotate=90] at ({\px-0.46},{\py+\ph/2})
    {Coverage $\uparrow$ (diversity)};

  % ---- one dot per model, colour is the only identifier -----------------
  % coordinates are the (MMD, Coverage) columns of section/tables_mean.tex
  \definecolor{mCNN}{HTML}{4C72B0}
  \definecolor{mLSTM}{HTML}{DD8452}
  \definecolor{mRNN}{HTML}{55A868}
  \definecolor{mWAVE}{HTML}{C44E52}
  \definecolor{mBEH}{HTML}{8172B3}
  \definecolor{mTRACE}{HTML}{937860}
  \definecolor{mRLP}{HTML}{DA8BC3}

  \foreach \m/\c/\col in {0.274/0.046/mCNN, 0.277/0.017/mLSTM, 0.460/0.018/mRNN,
                          0.130/0.254/mWAVE, 0.235/0.169/mBEH, 0.278/0.043/mTRACE,
                          0.435/0.010/mRLP} {
    \fill[\col] \pt{\m}{\c} circle (1.9pt);}

  % ---- CAG -------------------------------------------------------------
  \fill[cgBlue] \pt{0.041}{0.511} circle (2.6pt);
  \draw[draw=cgBlue, line width=0.5pt] \pt{0.041}{0.511} circle (4.2pt);

  % ---- legend: the upper-left corner is empty, so it costs no data -------
  \begin{scope}[shift={({\px+0.14},{\py+\ph-0.18})}]
    \foreach \i/\col/\name in {0/mCNN/CNN-GAN, 1/mLSTM/LSTM-GAN, 2/mRNN/RNN-GAN,
                               3/mWAVE/WaveGAN, 4/mBEH/BehaviorGAN,
                               5/mTRACE/TraceGAN, 6/mRLP/RLP-GAN} {
      \fill[\col] (0,{-\i*0.19}) circle (1.9pt);
      \node[font=\cgtiny, text=cgSlate, anchor=west, inner sep=2.4pt]
        at (0.06,{-\i*0.19}) {\name};}
    \fill[cgBlue] (0,{-7*0.19}) circle (2.2pt);
    \node[font=\cgtiny\bfseries, text=cgBlue!75!black, anchor=west, inner sep=2.4pt]
      at (0.06,{-7*0.19}) {CAG (ours)};
  \end{scope}

  \node[note, anchor=north west, text width=5.05cm] at (0.05,0.94)
    {Each baseline is accurate on one axis only. The lowest-MMD models stay below
     0.05 Coverage, and the highest-Coverage models stay above 0.13 MMD.
     CAG lies at MMD 0.041, Coverage 0.511.};
\end{scope}


==> figs/fig2/curves.tex <==
% Generated by code/scripts/fig2_data.py -- do not edit by hand.
% CoffeeMaker: routed "intermittent", K=6, cluster shares ['0.77', '0.14', '0.01', '0.01', '0.01', '0.06']
\newcommand{\routeinput}{\draw[trace] plot coordinates {(0.0000,0.0600) (0.0046,0.0600) (0.0091,0.0600) (0.0137,0.0600) (0.0183,0.0600) (0.0228,0.0600) (0.0274,0.0600) (0.0320,0.0600) (0.0365,0.0600) (0.0411,0.0600) (0.0457,0.0600) (0.0502,0.0600) (0.0548,0.0600) (0.0594,0.0600) (0.0639,0.0600) (0.0685,0.0600) (0.0731,0.0600) (0.0776,0.0600) (0.0822,0.0600) (0.0868,0.0600) (0.0913,0.0600) (0.0959,0.0600) (0.1005,0.0600) (0.1050,0.0600) (0.1096,0.0600) (0.1142,0.0600) (0.1187,0.0600) (0.1233,0.0600) (0.1279,0.0600) (0.1324,0.0600) (0.1370,0.0600) (0.1416,0.0600) (0.1461,0.0600) (0.1507,0.0600) (0.1553,0.0600) (0.1598,0.0600) (0.1644,0.0600) (0.1689,0.0600) (0.1735,0.0600) (0.1781,0.0600) (0.1826,0.0600) (0.1872,0.0600) (0.1918,0.0600) (0.1963,0.0600) (0.2009,0.0600) (0.2055,0.0600) (0.2100,0.0600) (0.2146,0.0600) (0.2192,0.0600) (0.2237,0.0600) (0.2283,0.0600) (0.2329,0.0600) (0.2374,0.0600) (0.2420,0.0600) (0.2466,0.0600) (0.2511,0.0600) (0.2557,0.8051) (0.2603,0.0600) (0.2648,0.0600) (0.2694,0.0600) (0.2740,0.0600) (0.2785,0.0600) (0.2831,0.0600) (0.2877,0.0600) (0.2922,0.0600) (0.2968,0.0600) (0.3014,0.0600) (0.3059,0.0600) (0.3105,0.0600) (0.3151,0.0600) (0.3196,0.0600) (0.3242,0.0600) (0.3288,0.0600) (0.3333,0.0600) (0.3379,0.0600) (0.3425,0.8147) (0.3470,0.0600) (0.3516,0.0600) (0.3562,0.0600) (0.3607,0.0600) (0.3653,0.0600) (0.3699,0.0600) (0.3744,0.0600) (0.3790,0.0600) (0.3836,0.0600) (0.3881,0.0600) (0.3927,0.0600) (0.3973,0.0600) (0.4018,0.0600) (0.4064,0.0600) (0.4110,0.0600) (0.4155,0.0600) (0.4201,0.0600) (0.4247,0.0600) (0.4292,0.8147) (0.4338,0.0600) (0.4384,0.0600) (0.4429,0.0600) (0.4475,0.0600) (0.4521,0.0600) (0.4566,0.0600) (0.4612,0.0600) (0.4658,0.0600) (0.4703,0.0600) (0.4749,0.0600) (0.4795,0.0600) (0.4840,0.0600) (0.4886,0.0600) (0.4932,0.0600) (0.4977,0.0600) (0.5023,0.0600) (0.5068,0.0600) (0.5114,0.8147) (0.5160,0.9400) (0.5205,0.0600) (0.5251,0.0600) (0.5297,0.0600) (0.5342,0.0600) (0.5388,0.0600) (0.5434,0.0600) (0.5479,0.0600) (0.5525,0.0600) (0.5571,0.0600) (0.5616,0.0600) (0.5662,0.0600) (0.5708,0.0600) (0.5753,0.0600) (0.5799,0.0600) (0.5845,0.0600) (0.5890,0.0600) (0.5936,0.0600) (0.5982,0.8147) (0.6027,0.9400) (0.6073,0.0600) (0.6119,0.0600) (0.6164,0.0600) (0.6210,0.0600) (0.6256,0.0600) (0.6301,0.0600) (0.6347,0.0600) (0.6393,0.0600) (0.6438,0.0600) (0.6484,0.0600) (0.6530,0.0600) (0.6575,0.0600) (0.6621,0.0600) (0.6667,0.0600) (0.6712,0.0600) (0.6758,0.0600) (0.6804,0.0600) (0.6849,0.9400) (0.6895,0.0600) (0.6941,0.0600) (0.6986,0.0600) (0.7032,0.0600) (0.7078,0.0600) (0.7123,0.0600) (0.7169,0.0600) (0.7215,0.0600) (0.7260,0.0600) (0.7306,0.0600) (0.7352,0.0600) (0.7397,0.0600) (0.7443,0.0600) (0.7489,0.0600) (0.7534,0.0600) (0.7580,0.0600) (0.7626,0.0600) (0.7671,0.8147) (0.7717,0.9400) (0.7763,0.0600) (0.7808,0.0600) (0.7854,0.0600) (0.7900,0.0600) (0.7945,0.0600) (0.7991,0.0600) (0.8037,0.0600) (0.8082,0.0600) (0.8128,0.0600) (0.8174,0.0600) (0.8219,0.0600) (0.8265,0.0600) (0.8311,0.0600) (0.8356,0.0600) (0.8402,0.0600) (0.8447,0.0600) (0.8493,0.0600) (0.8539,0.8147) (0.8584,0.9400) (0.8630,0.0600) (0.8676,0.0600) (0.8721,0.0600) (0.8767,0.0600) (0.8813,0.0600) (0.8858,0.0600) (0.8904,0.0600) (0.8950,0.0600) (0.8995,0.0600) (0.9041,0.0600) (0.9087,0.0600) (0.9132,0.0600) (0.9178,0.0600) (0.9224,0.0600) (0.9269,0.0600) (0.9315,0.0600) (0.9361,0.0600) (0.9406,0.9400) (0.9452,0.0600) (0.9498,0.0600) (0.9543,0.0600) (0.9589,0.0600) (0.9635,0.0600) (0.9680,0.0600) (0.9726,0.0600) (0.9772,0.0600) (0.9817,0.0600) (0.9863,0.0600) (0.9909,0.0600) (0.9954,0.0600) (1.0000,0.0600)};}
% cluster 1, 14% of windows
\newcommand{\clusta}{\draw[trace] plot coordinates {(0.0000,0.0955) (0.0105,0.0911) (0.0211,0.0919) (0.0316,0.0917) (0.0421,0.0897) (0.0526,0.0885) (0.0632,0.0883) (0.0737,0.0881) (0.0842,0.0893) (0.0947,0.0912) (0.1053,0.0883) (0.1158,0.0930) (0.1263,0.0908) (0.1368,0.0900) (0.1474,0.0881) (0.1579,0.0912) (0.1684,0.0920) (0.1789,0.0900) (0.1895,0.0893) (0.2000,0.0907) (0.2105,0.0888) (0.2211,0.0922) (0.2316,0.0909) (0.2421,0.0918) (0.2526,0.0901) (0.2632,0.0910) (0.2737,0.0922) (0.2842,0.0904) (0.2947,0.0905) (0.3053,0.0879) (0.3158,0.0903) (0.3263,0.0913) (0.3368,0.0890) (0.3474,0.0881) (0.3579,0.0887) (0.3684,0.0881) (0.3789,0.0881) (0.3895,0.0873) (0.4000,0.0918) (0.4105,0.0909) (0.4211,0.0880) (0.4316,0.0896) (0.4421,0.0912) (0.4526,0.0903) (0.4632,0.0854) (0.4737,0.0903) (0.4842,0.0863) (0.4947,0.0841) (0.5053,0.0824) (0.5158,0.0845) (0.5263,0.0866) (0.5368,0.0897) (0.5474,0.0859) (0.5579,0.0894) (0.5684,0.0875) (0.5789,0.0848) (0.5895,0.0849) (0.6000,0.0841) (0.6105,0.0881) (0.6211,0.0853) (0.6316,0.0853) (0.6421,0.0880) (0.6526,0.0881) (0.6632,0.0879) (0.6737,0.0881) (0.6842,0.0856) (0.6947,0.0888) (0.7053,0.0863) (0.7158,0.0870) (0.7263,0.0907) (0.7368,0.0872) (0.7474,0.0862) (0.7579,0.0853) (0.7684,0.0856) (0.7789,0.0871) (0.7895,0.0826) (0.8000,0.0866) (0.8105,0.0878) (0.8211,0.0893) (0.8316,0.0890) (0.8421,0.0905) (0.8526,0.0880) (0.8632,0.0876) (0.8737,0.0881) (0.8842,0.0863) (0.8947,0.0908) (0.9053,0.0864) (0.9158,0.0871) (0.9263,0.0892) (0.9368,0.0873) (0.9474,0.0890) (0.9579,0.0900) (0.9684,0.0862) (0.9789,0.0888) (0.9895,0.0875) (1.0000,0.0879)};}
% cluster 5, 6% of windows
\newcommand{\clustb}{\draw[trace] plot coordinates {(0.0000,0.1251) (0.0105,0.1187) (0.0211,0.1209) (0.0316,0.1321) (0.0421,0.1294) (0.0526,0.1318) (0.0632,0.1243) (0.0737,0.1186) (0.0842,0.1268) (0.0947,0.1291) (0.1053,0.1348) (0.1158,0.1361) (0.1263,0.1250) (0.1368,0.1357) (0.1474,0.1364) (0.1579,0.1273) (0.1684,0.1338) (0.1789,0.1311) (0.1895,0.1361) (0.2000,0.1301) (0.2105,0.1251) (0.2211,0.1383) (0.2316,0.1324) (0.2421,0.1225) (0.2526,0.1277) (0.2632,0.1227) (0.2737,0.1358) (0.2842,0.1385) (0.2947,0.1238) (0.3053,0.1319) (0.3158,0.1377) (0.3263,0.1262) (0.3368,0.1377) (0.3474,0.1291) (0.3579,0.1389) (0.3684,0.1349) (0.3789,0.1302) (0.3895,0.1341) (0.4000,0.1261) (0.4105,0.1196) (0.4211,0.1299) (0.4316,0.1235) (0.4421,0.1260) (0.4526,0.1241) (0.4632,0.1204) (0.4737,0.1323) (0.4842,0.1222) (0.4947,0.1245) (0.5053,0.1081) (0.5158,0.1175) (0.5263,0.1215) (0.5368,0.1274) (0.5474,0.1266) (0.5579,0.1300) (0.5684,0.1352) (0.5789,0.1344) (0.5895,0.1338) (0.6000,0.1343) (0.6105,0.1384) (0.6211,0.1380) (0.6316,0.1289) (0.6421,0.1352) (0.6526,0.1361) (0.6632,0.1341) (0.6737,0.1336) (0.6842,0.1378) (0.6947,0.1262) (0.7053,0.1283) (0.7158,0.1311) (0.7263,0.1294) (0.7368,0.1294) (0.7474,0.1265) (0.7579,0.1268) (0.7684,0.1252) (0.7789,0.1260) (0.7895,0.1144) (0.8000,0.1145) (0.8105,0.1187) (0.8211,0.1292) (0.8316,0.1215) (0.8421,0.1225) (0.8526,0.1262) (0.8632,0.1370) (0.8737,0.1312) (0.8842,0.1339) (0.8947,0.1349) (0.9053,0.1391) (0.9158,0.1310) (0.9263,0.1322) (0.9368,0.1300) (0.9474,0.1280) (0.9579,0.1309) (0.9684,0.1356) (0.9789,0.1284) (0.9895,0.1332) (1.0000,0.1343)};}
% cluster 2, 1% of windows
\newcommand{\clustc}{\draw[trace] plot coordinates {(0.0000,0.0960) (0.0105,0.1402) (0.0211,0.1297) (0.0316,0.1196) (0.0421,0.0851) (0.0526,0.1061) (0.0632,0.1508) (0.0737,0.1937) (0.0842,0.1348) (0.0947,0.0846) (0.1053,0.1156) (0.1158,0.0878) (0.1263,0.1187) (0.1368,0.1072) (0.1474,0.1061) (0.1579,0.1038) (0.1684,0.1030) (0.1789,0.1108) (0.1895,0.1168) (0.2000,0.1411) (0.2105,0.0839) (0.2211,0.0935) (0.2316,0.1250) (0.2421,0.1207) (0.2526,0.1070) (0.2632,0.1312) (0.2737,0.1039) (0.2842,0.0819) (0.2947,0.1006) (0.3053,0.1038) (0.3158,0.0948) (0.3263,0.1034) (0.3368,0.1110) (0.3474,0.1035) (0.3579,0.1198) (0.3684,0.1009) (0.3789,0.1387) (0.3895,0.1137) (0.4000,0.1235) (0.4105,0.1641) (0.4211,0.1418) (0.4316,0.1263) (0.4421,0.1413) (0.4526,0.1553) (0.4632,0.1615) (0.4737,0.1530) (0.4842,0.1899) (0.4947,0.2669) (0.5053,0.7600) (0.5158,0.2568) (0.5263,0.2198) (0.5368,0.1562) (0.5474,0.1366) (0.5579,0.1516) (0.5684,0.1429) (0.5789,0.1063) (0.5895,0.1817) (0.6000,0.1233) (0.6105,0.0921) (0.6211,0.1028) (0.6316,0.1255) (0.6421,0.1111) (0.6526,0.0959) (0.6632,0.1246) (0.6737,0.1609) (0.6842,0.0922) (0.6947,0.0844) (0.7053,0.1184) (0.7158,0.1231) (0.7263,0.1154) (0.7368,0.1047) (0.7474,0.1252) (0.7579,0.1155) (0.7684,0.1141) (0.7789,0.1302) (0.7895,0.1061) (0.8000,0.1404) (0.8105,0.1420) (0.8211,0.1018) (0.8316,0.1310) (0.8421,0.1573) (0.8526,0.1169) (0.8632,0.1130) (0.8737,0.1048) (0.8842,0.0925) (0.8947,0.1199) (0.9053,0.1022) (0.9158,0.1010) (0.9263,0.1594) (0.9368,0.1015) (0.9474,0.1215) (0.9579,0.1422) (0.9684,0.1039) (0.9789,0.1300) (0.9895,0.1055) (1.0000,0.1146)};}
% WaterCooler: envelope aggregation factor r=8 (512 -> 64 points)
\newcommand{\contraw}{\draw[trace] plot coordinates {(0.0000,0.1901) (0.0105,0.1901) (0.0211,0.1901) (0.0316,0.9037) (0.0421,0.9037) (0.0526,0.9056) (0.0632,0.1901) (0.0737,0.1901) (0.0842,0.1901) (0.0947,0.1901) (0.1053,0.1901) (0.1158,0.1901) (0.1263,0.1901) (0.1368,0.9017) (0.1474,0.8998) (0.1579,0.8989) (0.1684,0.8979) (0.1789,0.1901) (0.1895,0.1901) (0.2000,0.1901) (0.2105,0.1901) (0.2211,0.1901) (0.2316,0.1901) (0.2421,0.1901) (0.2526,0.9017) (0.2632,0.8979) (0.2737,0.8979) (0.2842,0.8941) (0.2947,0.1901) (0.3053,0.1901) (0.3158,0.1901) (0.3263,0.1901) (0.3368,0.1901) (0.3474,0.1901) (0.3579,0.1901) (0.3684,0.9151) (0.3789,0.9151) (0.3895,0.9113) (0.4000,0.9113) (0.4105,0.1901) (0.4211,0.1901) (0.4316,0.1901) (0.4421,0.1901) (0.4526,0.1901) (0.4632,0.1901) (0.4737,0.1901) (0.4842,0.9132) (0.4947,0.9094) (0.5053,0.9094) (0.5158,0.9094) (0.5263,0.1901) (0.5368,0.1901) (0.5474,0.1901) (0.5579,0.1901) (0.5684,0.1901) (0.5789,0.1901) (0.5895,0.1901) (0.6000,0.9094) (0.6105,0.9075) (0.6211,0.9075) (0.6316,0.9056) (0.6421,0.1901) (0.6526,0.1901) (0.6632,0.1901) (0.6737,0.1901) (0.6842,0.1901) (0.6947,0.1901) (0.7053,0.1901) (0.7158,0.9056) (0.7263,0.9037) (0.7368,0.9056) (0.7474,0.9037) (0.7579,0.1901) (0.7684,0.1901) (0.7789,0.1901) (0.7895,0.1901) (0.8000,0.1901) (0.8105,0.1901) (0.8211,0.1901) (0.8316,0.9075) (0.8421,0.9056) (0.8526,0.9017) (0.8632,0.9017) (0.8737,0.1901) (0.8842,0.1901) (0.8947,0.1901) (0.9053,0.1901) (0.9158,0.1901) (0.9263,0.1901) (0.9368,0.1901) (0.9474,0.9094) (0.9579,0.9037) (0.9684,0.9017) (0.9789,0.9017) (0.9895,0.1901) (1.0000,0.1901)};}
\newcommand{\contenv}{\draw[trace] plot coordinates {(0.0000,0.1901) (0.0159,0.1901) (0.0317,0.9032) (0.0476,0.5466) (0.0635,0.1901) (0.0794,0.1901) (0.0952,0.1898) (0.1111,0.1896) (0.1270,0.6193) (0.1429,0.8984) (0.1587,0.3670) (0.1746,0.1898) (0.1905,0.1901) (0.2063,0.1894) (0.2222,0.1901) (0.2381,0.7217) (0.2540,0.8967) (0.2698,0.2769) (0.2857,0.1898) (0.3016,0.1889) (0.3175,0.1898) (0.3333,0.1901) (0.3492,0.7322) (0.3651,0.9094) (0.3810,0.2802) (0.3968,0.1901) (0.4127,0.1901) (0.4286,0.1901) (0.4444,0.1901) (0.4603,0.9099) (0.4762,0.9080) (0.4921,0.1901) (0.5079,0.1901) (0.5238,0.1901) (0.5397,0.1901) (0.5556,0.1901) (0.5714,0.8166) (0.5873,0.7269) (0.6032,0.1901) (0.6190,0.1901) (0.6349,0.1901) (0.6508,0.1901) (0.6667,0.4546) (0.6825,0.9029) (0.6984,0.5471) (0.7143,0.1901) (0.7302,0.1901) (0.7460,0.1901) (0.7619,0.1896) (0.7778,0.5488) (0.7937,0.9032) (0.8095,0.6349) (0.8254,0.1901) (0.8413,0.1901) (0.8571,0.1901) (0.8730,0.1901) (0.8889,0.6355) (0.9048,0.9008) (0.9206,0.4565) (0.9365,0.1901) (0.9524,0.1901) (0.9683,0.1898) (0.9841,0.1901) (1.0000,0.6540)};}
\newcommand{\contrec}{\draw[trace] plot coordinates {(0.0000,0.1901) (0.0079,0.1901) (0.0157,0.1901) (0.0236,0.1901) (0.0315,0.9032) (0.0394,0.9032) (0.0472,0.5466) (0.0551,0.5466) (0.0630,0.1901) (0.0709,0.1901) (0.0787,0.1901) (0.0866,0.1901) (0.0945,0.1898) (0.1024,0.1898) (0.1102,0.1896) (0.1181,0.1896) (0.1260,0.6193) (0.1339,0.6193) (0.1417,0.8984) (0.1496,0.8984) (0.1575,0.3670) (0.1654,0.3670) (0.1732,0.1898) (0.1811,0.1898) (0.1890,0.1901) (0.1969,0.1901) (0.2047,0.1894) (0.2126,0.1894) (0.2205,0.1901) (0.2283,0.1901) (0.2362,0.7217) (0.2441,0.7217) (0.2520,0.8967) (0.2598,0.8967) (0.2677,0.2769) (0.2756,0.2769) (0.2835,0.1898) (0.2913,0.1898) (0.2992,0.1889) (0.3071,0.1889) (0.3150,0.1898) (0.3228,0.1898) (0.3307,0.1901) (0.3386,0.1901) (0.3465,0.7322) (0.3543,0.7322) (0.3622,0.9094) (0.3701,0.9094) (0.3780,0.2802) (0.3858,0.2802) (0.3937,0.1901) (0.4016,0.1901) (0.4094,0.1901) (0.4173,0.1901) (0.4252,0.1901) (0.4331,0.1901) (0.4409,0.1901) (0.4488,0.1901) (0.4567,0.9099) (0.4646,0.9099) (0.4724,0.9080) (0.4803,0.9080) (0.4882,0.1901) (0.4961,0.1901) (0.5039,0.1901) (0.5118,0.1901) (0.5197,0.1901) (0.5276,0.1901) (0.5354,0.1901) (0.5433,0.1901) (0.5512,0.1901) (0.5591,0.1901) (0.5669,0.8166) (0.5748,0.8166) (0.5827,0.7269) (0.5906,0.7269) (0.5984,0.1901) (0.6063,0.1901) (0.6142,0.1901) (0.6220,0.1901) (0.6299,0.1901) (0.6378,0.1901) (0.6457,0.1901) (0.6535,0.1901) (0.6614,0.4546) (0.6693,0.4546) (0.6772,0.9029) (0.6850,0.9029) (0.6929,0.5471) (0.7008,0.5471) (0.7087,0.1901) (0.7165,0.1901) (0.7244,0.1901) (0.7323,0.1901) (0.7402,0.1901) (0.7480,0.1901) (0.7559,0.1896) (0.7638,0.1896) (0.7717,0.5488) (0.7795,0.5488) (0.7874,0.9032) (0.7953,0.9032) (0.8031,0.6349) (0.8110,0.6349) (0.8189,0.1901) (0.8268,0.1901) (0.8346,0.1901) (0.8425,0.1901) (0.8504,0.1901) (0.8583,0.1901) (0.8661,0.1901) (0.8740,0.1901) (0.8819,0.6355) (0.8898,0.6355) (0.8976,0.9008) (0.9055,0.9008) (0.9134,0.4565) (0.9213,0.4565) (0.9291,0.1901) (0.9370,0.1901) (0.9449,0.1901) (0.9528,0.1901) (0.9606,0.1898) (0.9685,0.1898) (0.9764,0.1901) (0.9843,0.1901) (0.9921,0.6540) (1.0000,0.6540)};}
\newcommand{\cagout}{\draw[trace] plot coordinates {(0.0000,0.1007) (0.0105,0.0602) (0.0211,0.0600) (0.0316,0.6011) (0.0421,0.2930) (0.0526,0.7682) (0.0632,0.1826) (0.0737,0.0666) (0.0842,0.4104) (0.0947,0.2775) (0.1053,0.2193) (0.1158,0.1103) (0.1263,0.0636) (0.1368,0.3777) (0.1474,0.0651) (0.1579,0.2843) (0.1684,0.0637) (0.1789,0.1363) (0.1895,0.7685) (0.2000,0.0610) (0.2105,0.0740) (0.2211,0.1684) (0.2316,0.7026) (0.2421,0.2456) (0.2526,0.6140) (0.2632,0.3922) (0.2737,0.3903) (0.2842,0.0608) (0.2947,0.0611) (0.3053,0.8036) (0.3158,0.8641) (0.3263,0.6761) (0.3368,0.0685) (0.3474,0.1547) (0.3579,0.6447) (0.3684,0.3802) (0.3789,0.3896) (0.3895,0.8573) (0.4000,0.0619) (0.4105,0.9125) (0.4211,0.1037) (0.4316,0.1180) (0.4421,0.7831) (0.4526,0.9394) (0.4632,0.8166) (0.4737,0.1969) (0.4842,0.0728) (0.4947,0.0832) (0.5053,0.0690) (0.5158,0.0838) (0.5263,0.1862) (0.5368,0.0823) (0.5474,0.1381) (0.5579,0.4881) (0.5684,0.0652) (0.5789,0.7757) (0.5895,0.0638) (0.6000,0.2837) (0.6105,0.1009) (0.6211,0.0639) (0.6316,0.0601) (0.6421,0.0600) (0.6526,0.0607) (0.6632,0.6035) (0.6737,0.0600) (0.6842,0.0831) (0.6947,0.7148) (0.7053,0.2701) (0.7158,0.0601) (0.7263,0.0605) (0.7368,0.0924) (0.7474,0.6502) (0.7579,0.0628) (0.7684,0.0600) (0.7789,0.0959) (0.7895,0.0800) (0.8000,0.3715) (0.8105,0.0648) (0.8211,0.0661) (0.8316,0.0622) (0.8421,0.0656) (0.8526,0.0605) (0.8632,0.0626) (0.8737,0.0600) (0.8842,0.9336) (0.8947,0.0607) (0.9053,0.0600) (0.9158,0.0691) (0.9263,0.0774) (0.9368,0.1108) (0.9474,0.0814) (0.9579,0.0600) (0.9684,0.0629) (0.9789,0.2531) (0.9895,0.0645) (1.0000,0.0718)};}


==> figs/fig2/panel_a.tex <==
% ---------------------------------------------------------------------
% Fig. 2 (a): behavioural routing. The trace and the duty cycle are real
% (code/scripts/fig2_data.py); rho and the ON level are the constants in
% cagbench/models/cag.py. Local frame: bottom-left, 3.05 x 5.40 units.
% ---------------------------------------------------------------------
\begin{scope}
  \node[ptitle] at (0,5.22) {(a) Routing};
  \node[psub]   at (0,4.98) {one decision per appliance};

  \draw[well] (0.02,4.06) rectangle (3.00,4.72);
  \begin{scope}\clip (0.02,4.06) rectangle (3.00,4.72);
    \begin{scope}[shift={(0.02,4.06)}, x=2.98cm, y=0.66cm] \routeinput \end{scope}
  \end{scope}
  \node[psub] at (0.02,3.90) {measured active power};

  % one label per card, centred in its own card
  \foreach \i/\t in {0/{$x^{(1)}$}, 1/{$x^{(2)}$}, 2/{$\cdots$}}{
    \draw[card] ({0.14+\i*0.98},3.20) rectangle ({1.02+\i*0.98},3.60);
    \node[lab] at ({0.58+\i*0.98},3.40) {\t};}
  \node[psub] at (0.02,3.02) {windows of $L=436$};

  \node[chipN, anchor=north west, align=left] at (0.02,2.76)
    {$d=\frac{1}{NL}\sum_{n,t}\mathbf{1}[x^{(n)}_t>\theta]$};
  \draw[flow] (1.51,2.28) -- (1.51,2.04);
  \node[card, anchor=north, minimum width=1.9cm, minimum height=0.30cm,
        font=\cgtiny, inner sep=2pt] at (1.51,2.04) {$d>\rho=0.7$ ?};

  % the two branch colours are fixed here and used for the rest of the figure
  \draw[flowG] (2.51,1.80) -- (3.02,1.80) node[midway, above, font=\cgtiny] {yes};
  \draw[flowB] (0.51,1.80) -- (0.51,1.16) -- (3.02,1.16);
  \node[font=\cgtiny, text=cgBlue, anchor=south west] at (0.55,1.18) {no};
  \node[chipG, anchor=east] at (2.48,1.46) {continuous};
  \node[chipB, anchor=west] at (0.60,0.88) {intermittent};
  \node[note, anchor=north west, text width=3.00cm] at (0.02,0.62)
    {Four appliances are always on; the other seven are event driven.};
\end{scope}


==> figs/fig2/panel_b.tex <==
% ---------------------------------------------------------------------
% Fig. 2 (b): intermittent branch. Cluster count, shares and centroid
% shapes are the real output of cluster_segments() on CoffeeMaker
% (code/scripts/fig2_data.py). Local frame: bottom-left, 7.80 x 3.05.
% ---------------------------------------------------------------------
\begin{scope}
  \node[ptitle] at (0,2.86) {(b) Intermittent branch};
  \node[psub]   at (0,2.62) {one generator per operating state};

  % ---- operating-state clustering --------------------------------------
  \foreach \i/\m/\s in {0/\clusta/{14\%}, 1/\clustb/{6\%}, 2/\clustc/{1\%}} {
    \pgfmathsetmacro{\x}{0.02+\i*0.80}
    \draw[well] (\x,1.72) rectangle ({\x+0.72},2.42);
    \begin{scope}\clip (\x,1.72) rectangle ({\x+0.72},2.42);
      \begin{scope}[shift={(\x,1.72)}, x=0.72cm, y=0.70cm,
                    trace/.append style={draw=cgBlue}] \m \end{scope}
    \end{scope}
    \node[font=\cgtiny, text=cgSlate, anchor=north east, inner sep=1.6pt]
      at ({\x+0.72},2.42) {\s};}
  \node[chipN, anchor=north west] at (0.02,1.62) {idle cluster, 77\%};
  \node[note, anchor=north west, text width=2.30cm] at (0.02,1.30)
    {$k$-means on shape descriptors, $K=6$ by silhouette; the idle share is
     the appliance's duty cycle};

  % ---- per-cluster generators ------------------------------------------
  \draw[flowB] (2.44,2.07) -- (2.72,2.07);
  \foreach \i in {0,1,2}{
    \draw[cardB] ({2.78+\i*0.08},{1.80+\i*0.08}) rectangle ({3.84+\i*0.08},{2.28+\i*0.08});}
  % the stack is drawn back to front; the label belongs on the front card
  \node[lab] at (3.47,2.20) {$G_k(z,k)$};
  \node[chipN, anchor=north west] at (2.78,1.62) {$z\sim\mathcal{N}(0,I)$};

  % ---- discriminator and objective -------------------------------------
  \draw[flowB] (4.00,2.07) -- (4.16,2.07);
  \node[cardB, anchor=west, minimum width=1.25cm, minimum height=0.54cm,
        font=\cgtiny, align=center] at (4.16,2.07) {$D_k$, multi-\\resolution};
  \draw[flowB] (5.48,2.07) -- (5.66,2.07);
  \node[chipB, anchor=west] at (5.66,2.07) {real vs. fake};
  \node[chipA, anchor=north west] at (5.66,1.86) {EMA + shift aug.};
  % the measured windows of the same cluster are D's other input
  \draw[flow, draw=cgSlate] (2.44,1.30) -- (4.58,1.30) -- (4.58,1.78);
  \node[psub, anchor=west] at (2.78,1.18) {measured windows of cluster $k$};
\end{scope}


==> figs/fig2/panel_c.tex <==
% ---------------------------------------------------------------------
% Fig. 2 (c): continuous branch. The raw window, its envelope and the
% reconstruction are one WaterCooler window through the block average of
% Eq. (avg-simplify), r=8. Local frame: bottom-left, 7.80 x 2.05 units.
% ---------------------------------------------------------------------
\begin{scope}
  \node[ptitle] at (0,1.88) {(c) Continuous branch};
  \node[psub]   at (3.70,1.88) {model the envelope, then reconstruct};

  \foreach \i/\m/\t in {0/\contraw/{full rate, $T$},
                        1/\contenv/{envelope, $T/r$, $r=8$}} {
    \pgfmathsetmacro{\x}{0.02+\i*2.06}
    \draw[well] (\x,0.80) rectangle ({\x+1.60},1.36);
    \begin{scope}\clip (\x,0.80) rectangle ({\x+1.60},1.36);
      \begin{scope}[shift={(\x,0.80)}, x=1.60cm, y=0.56cm,
                    trace/.append style={draw=cgGreen}] \m \end{scope}
    \end{scope}
    \node[font=\cgtiny, text=cgSlate, anchor=north] at ({\x+0.80},0.78) {\t};}
  \draw[flowG] (1.68,1.08) -- (2.02,1.08);
  \node[font=\cgtiny, text=cgSlate, anchor=south, inner sep=1pt]
    at (1.85,1.40) {$\bar{x}_j=\frac{1}{r}\sum_{t\in b_j}x_t$};

  \draw[flowG] (3.72,1.08) -- (4.00,1.08);
  \node[cardG, anchor=west, minimum width=1.0cm, minimum height=0.50cm,
        font=\cgtiny, align=center] at (4.00,1.08) {LSTM\\$G$, $D$};
  \draw[flowG] (5.16,1.08) -- (5.48,1.08);
  \node[font=\cgtiny, text=cgSlate, anchor=south, inner sep=1pt]
    at (5.32,1.40) {repeat $r$};

  \draw[well] (5.54,0.80) rectangle (7.14,1.36);
  \begin{scope}\clip (5.54,0.80) rectangle (7.14,1.36);
    \begin{scope}[shift={(5.54,0.80)}, x=1.60cm, y=0.56cm,
                  trace/.append style={draw=cgGreen}] \contrec \end{scope}
  \end{scope}
  \node[font=\cgtiny, text=cgSlate, anchor=north] at (6.34,0.78) {reconstructed};
  \node[note, anchor=north west, text width=7.55cm] at (0.02,0.46)
    {Aggregation removes the sample-to-sample redundancy of an always-on appliance, so the
     recurrent model is trained on the operating envelope rather than on sample-level noise.};
\end{scope}


==> figs/fig2/panel_d.tex <==
% ---------------------------------------------------------------------
% Fig. 2 (d): what comes out. The trace is a real sample from the trained
% CoffeeMaker generator (results/final/CAG_A_s0_p0_CoffeeMaker.npy).
% Local frame: bottom-left, 4.65 x 5.40 units.
% ---------------------------------------------------------------------
\begin{scope}
  \node[ptitle] at (0,5.22) {(d) Synthesised profile};
  \node[psub]   at (0,4.98) {a sample from the trained generator};

  \draw[well] (0.02,4.06) rectangle (4.60,4.72);
  \begin{scope}\clip (0.02,4.06) rectangle (4.60,4.72);
    \begin{scope}[shift={(0.02,4.06)}, x=4.58cm, y=0.66cm,
                  trace/.append style={draw=cgBlue}] \cagout \end{scope}
  \end{scope}

  \node[note, anchor=north west, text width=4.55cm] at (0.02,3.90)
    {Cluster samples are drawn in proportion to the measured cluster shares and
     concatenated, so the synthesised profile carries the appliance's duty cycle
     as well as the shape of each operating state.};

  \node[lab, anchor=north west, font=\cgsmall\bfseries] at (0.02,2.34) {Downstream use};
  \foreach \i/\t in {0/{NILM training data}, 1/{data augmentation},
                     2/{privacy-preserving sharing}} {
    \node[chipN, anchor=north west] at (0.02,{2.04-\i*0.38}) {\t};}
\end{scope}


==> figs/fig2/panel_e.tex <==
% ---------------------------------------------------------------------
% Fig. 2 (e): the per-device adaptive components. Which one a device gets
% is decided per appliance; the ablation table measures what they add, so
% no counts are repeated here.
% Local frame: origin at bottom-left, 16.0 x 1.90 units.
% ---------------------------------------------------------------------
\begin{scope}
  \draw[panel] (0,0) rectangle (16.0,1.90);
  \node[ptitle, anchor=west] at (0.22,1.62) {(e) Per-device adaptive components};
  \node[psub, anchor=west] at (5.60,1.62)
    {selected per appliance; the ablation in Table~\ref{tab:ablation-study} isolates their effect};
  \foreach \i/\n/\t in {%
      0/{behaviour-factorised $G$}/{a Gumbel-sigmoid switch separates on/off activity from power
         magnitude --- fixes event statistics},
      1/{marginal moment matching}/{penalises the gap between generated and measured power mean
         and standard deviation --- fixes power-level bias},
      2/{dilated convolution stack}/{widens the receptive field of the per-cluster generator ---
         fixes long-range spectral structure},
      3/{generator blending}/{mixes a cluster-specific and a waveform-transposed generator, so
         two architectures can contribute}} {
    \pgfmathsetmacro{\x}{0.30+\i*3.92}
    \node[chipA, anchor=north west, font=\cgtiny\bfseries] at (\x,1.34) {\n};
    \node[note, anchor=north west, text width=3.55cm] at (\x,0.98) {\t};}
\end{scope}

